C-RAN with Hybrid RF/FSO Fronthaul Links: Joint Optimization of RF Time Allocation and Fronthaul Compression

This paper considers the uplink of a cloud radio access network (C-RAN) comprised of several multi-antenna remote radio units (RUs) which send the data that they received from multiple mobile users (MUs) to a central unit (CU) via a wireless fronthaul link. One of the fundamental challenges in implementing C-RAN is the huge data rate required for fronthauling. To address this issue, we employ hybrid radio frequency (RF)/free space optical (FSO) systems for the fronthaul links as they benefit from both the large data rates of FSO links and the reliability of RF links. To efficiently exploit the fronthaul capacity, the RUs employ vector quantization to jointly compress the signals received at their antennas. Moreover, due to the limited available RF spectrum, we assume that the RF multiple-access and fronthaul links employ the same RF resources. Thereby, we propose an adaptive protocol which allocates transmission time to the RF multiple-access and fronthaul links in a time division duplex (TDD) manner and optimizes the quantization noise covariance matrix at each RU such that the sum rate is maximized. Our simulation results reveal that a considerable gain in terms of sum rate can be achieved by the proposed protocol in comparison with benchmark schemes from the literature, especially when the FSO links experience unfavorable atmospheric conditions.

==> Fig/Fig1/Rate_Alpha.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{022}[bc][bc]{\matlabtextA $C_{\mathrm{sum}}$ (Mbps)}%
\psfrag{023}[tc][tc]{\matlabtextA $\alpha_0$}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{12}{12}\selectfont\strut}%
\psfrag{021}[cl][cl]{\matlabtextB $\kappa=10^{-3}*[0.43, 60, 75, 100]$}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextC{\color[rgb]{0.000,0.000,0.000}\fontsize{8}{8}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextC $0$}%
\psfrag{001}[ct][ct]{\matlabtextC $0.1$}%
\psfrag{002}[ct][ct]{\matlabtextC $0.2$}%
\psfrag{003}[ct][ct]{\matlabtextC $0.3$}%
\psfrag{004}[ct][ct]{\matlabtextC $0.4$}%
\psfrag{005}[ct][ct]{\matlabtextC $0.5$}%
\psfrag{006}[ct][ct]{\matlabtextC $0.6$}%
\psfrag{007}[ct][ct]{\matlabtextC $0.7$}%
\psfrag{008}[ct][ct]{\matlabtextC $0.8$}%
\psfrag{009}[ct][ct]{\matlabtextC $0.9$}%
\psfrag{010}[ct][ct]{\matlabtextC $1$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{011}[rc][rc]{\matlabtextC $0$}%
\psfrag{012}[rc][rc]{\matlabtextC $200$}%
\psfrag{013}[rc][rc]{\matlabtextC $400$}%
\psfrag{014}[rc][rc]{\matlabtextC $600$}%
\psfrag{015}[rc][rc]{\matlabtextC $800$}%
\psfrag{016}[rc][rc]{\matlabtextC $1000$}%
\psfrag{017}[rc][rc]{\matlabtextC $1200$}%
\psfrag{018}[rc][rc]{\matlabtextC $1400$}%
\psfrag{019}[rc][rc]{\matlabtextC $1600$}%
\psfrag{020}[rc][rc]{\matlabtextC $1800$}%
%
%% </ytick>

==> Fig/Fig3/Rate_dfrhl.tex <==
% Generated using matlabfrag
% Version: v0.6.16
% Version Date: 04-Apr-2010
% Author: Zebb Prime
%
%% <text>
%
\providecommand\matlabtextA{\color[rgb]{0.000,0.000,0.000}\fontsize{9}{9}\selectfont\strut}%
\psfrag{022}[cl][cl]{\matlabtextA $\kappa=125*10^{-3}$\hspace{0.5em}}%
\psfrag{023}[cl][cl]{\matlabtextA $\kappa=42*10^{-3}$\hspace{0.5em}}%
\psfrag{024}[cl][cl]{\matlabtextA $\kappa=4.2*10^{-3}$\hspace{0.5em}}%
\psfrag{030}[cl][cl]{\matlabtextA FSO-SQ\hspace{0.5em}}%
\psfrag{031}[cl][cl]{\matlabtextA FSO-VQ\hspace{0.5em}}%
\psfrag{032}[cl][cl]{\matlabtextA Proposed Hybrid RF/FSO-VQ\hspace{0.5em}}%
%
\providecommand\matlabtextB{\color[rgb]{0.000,0.000,0.000}\fontsize{10}{10}\selectfont\strut}%
\psfrag{033}[bc][bc]{\matlabtextB $C_{\mathrm{sum}}$ (Mbps)}%
\psfrag{034}[tc][tc]{\matlabtextB $d^{\mathrm{fr}}$ (m)}%
%
\providecommand\matlabtextC{\color[rgb]{0.000,0.000,0.000}\fontsize{12}{12}\selectfont\strut}%
\psfrag{025}[cl][cl]{\matlabtextC gain}%
\psfrag{026}[cl][cl]{\matlabtextC Mbps}%
\psfrag{027}[cl][cl]{\matlabtextC 230}%
\psfrag{028}[cl][cl]{\matlabtextC 650 Mbps gain}%
\psfrag{029}[cl][cl]{\matlabtextC 160 Mbps gain}%
%
%% </text>
%
%% <xtick>
%
\def\matlabfragNegXTick{\mathord{\makebox[0pt][r]{$-$}}}
%
\providecommand\matlabtextD{\color[rgb]{0.000,0.000,0.000}\fontsize{8}{8}\selectfont\strut}%
\psfrag{000}[ct][ct]{\matlabtextD $100$}%
\psfrag{001}[ct][ct]{\matlabtextD $200$}%
\psfrag{002}[ct][ct]{\matlabtextD $300$}%
\psfrag{003}[ct][ct]{\matlabtextD $400$}%
\psfrag{004}[ct][ct]{\matlabtextD $500$}%
\psfrag{005}[ct][ct]{\matlabtextD $600$}%
\psfrag{006}[ct][ct]{\matlabtextD $700$}%
\psfrag{007}[ct][ct]{\matlabtextD $800$}%
\psfrag{008}[ct][ct]{\matlabtextD $900$}%
\psfrag{009}[ct][ct]{\matlabtextD $1000$}%
%
%% </xtick>
%
%% <ytick>
%
\psfrag{010}[rc][rc]{\matlabtextD $0$}%
\psfrag{011}[rc][rc]{\matlabtextD $200$}%
\psfrag{012}[rc][rc]{\matlabtextD $400$}%
\psfrag{013}[rc][rc]{\matlabtextD $600$}%
\psfrag{014}[rc][rc]{\matlabtextD $800$}%
\psfrag{015}[rc][rc]{\matlabtextD $1000$}%
\psfrag{016}[rc][rc]{\matlabtextD $1200$}%
\psfrag{017}[rc][rc]{\matlabtextD $1400$}%
\psfrag{018}[rc][rc]{\matlabtextD $1600$}%
\psfrag{019}[rc][rc]{\matlabtextD $1800$}%
\psfrag{020}[rc][rc]{\matlabtextD $2000$}%
\psfrag{021}[rc][rc]{\matlabtextD $2200$}%
%
%% </ytick>
